Census of the Local Universe (CLU) Narrow-Band Survey I: Galaxy Catalogs from Preliminary Fields

We present the Census of the Local Universe (CLU) narrow-band survey to search for emission-line (\ha) galaxies. CLU-\ha~has imaged $\approx$3$\pi$ of the sky (26,470~deg$^2$) with 4 narrow-band filters that probe a distance out to 200~Mpc. We have obtained spectroscopic follow-up for galaxy candidates in 14 preliminary fields (101.6~deg$^2$) to characterize the limits and completeness of the survey. In these preliminary fields, CLU can identify emission lines down to an \ha~flux limit of $10^{-14}$~$\rm{erg~s^{-1}~cm^{-2}}$ at 90\% completeness, and recovers 83\% (67\%) of the \ha~flux from catalogued galaxies in our search volume at the $\Sigma$=2.5 ($\Sigma$=5) color excess levels. The contamination from galaxies with no emission lines is 61\% (12\%) for $\Sigma$=2.5 ($\Sigma$=5). Also, in the regions of overlap between our preliminary fields and previous emission-line surveys, we recover the majority of the galaxies found in previous surveys and identify an additional $\approx$300 galaxies. In total, we find 90 galaxies with no previous distance information, several of which are interesting objects: 7 blue compact dwarfs, 1 green pea, and a Seyfert galaxy; we also identified a known planetary nebula. These objects show that the CLU-\ha~survey can be a discovery machine for objects in our own Galaxy and extreme galaxies out to intermediate redshifts. However, the majority of the CLU-\ha~galaxies identified in this work show properties consistent with normal star-forming galaxies. CLU-\ha~galaxies with new redshifts will be added to existing galaxy catalogs to focus the search for the electromagnetic counterpart to gravitational wave events.

==> tables/completeness.tex <==
\begin{table*}
\begin{center}
{Completeness}\\
\begin{tabular}{cccccc}
\hline
\hline

Catalog			& N 		& Sum Lum (B)	& Sum Lum (\ha)	&Sum \ha~SFR	& Log Sum Mstar	\\
			&Vol Corrected	&Vol Corrected	&Vol Corrected	&Vol Corrected	&Vol Corrected	\\
(\#)			& (\#)		& (\#)		& (\#)		& (\#)		& (\#)		\\
\hline
LVL			& 2046.80	&9.0118891e+45	&2.8535251e+43	&383.280	&1.02024e+13	\\
All SDSS		& 1116.72	&1.2193141e+46	&7.8652492e+42	&253.36571	&1.0842249e+13	\\
SDSS Prelim		& 1186		&1.2314988e+46	&3.8021326e+42	&253.07957	&1.0717518e+13	\\
$\Sigma=2.5$		& 246		&2.7588785e+45	&2.9213481e+42	&189.11595	&2.3988876e+12	\\  
$\Sigma=5.0$		& 128		&1.5824658e+45	&2.2129135e+42	&143.63836	&1.5026702e+12	\\
\hline
SDSS Prelim+CLU-new	& 1264		&1.2826438e+46	&4.6870528e+42	&283.85251	&1.1117338e+13
	\\
\hline
\end{tabular}\\
\end{center}
\caption{\textbf{DC: very outdated...still working on this...}}
\label{tab:complete}
\end{table*}



==> tables/knowngal.tex <==
\begin{table*}
\begin{center}
{Known Galaxies}\\
\begin{tabular}{ccccccc}
\hline
\hline

Sample		&\vline& N			& Sum \ha~Flux			&\vline& N (EW $>$ 7.5~\AA)	& Sum \ha~Flux (EW $>$ 7.5~\AA)	      \\
		&\vline&(\#,\% of N)		& (erg/s/cm$^2$,\% of Flux)	&\vline& (\#,\% of N)		& (erg/s/cm$^2$,\% of Flux)	      \\
\hline
All 		&\vline& 1226			& 4.15e-12		&\vline& 504			& 3.89e-12		      \\
\hline
$\Sigma=2.5$	&\vline&297~(24.2\%)	&3.36e-12~(80.9\%)		&\vline&262~(52.0\%)		&3.32e-12~(85.2\%)		\\  
3.0		&\vline&261~(21.3\%)	&3.26e-12~(78.4\%)		&\vline&234~(46.4\%)		&3.22e-12~(82.7\%)	    \\
4.0		&\vline&194~(15.8\%)	&2.96e-12~(71.1\%)		&\vline&181~(35.9\%)		&2.95e-12~(75.7\%)	    \\
5.0		&\vline&152~(12.4\%)	&2.76e-12~(66.4\%)		&\vline&143~(28.4\%)		&2.75e-12~(70.7\%)	    \\
6.0		&\vline&121~(~9.9\%)	&2.57e-12~(61.9\%)		&\vline&113~(22.4\%)		&2.57e-12~(65.9\%)	    \\
7.0		&\vline&103~(~8.4\%)	&2.35e-12~(56.6\%)		&\vline& 97~(19.2\%)		&2.35e-12~(60.4\%)	    \\
\hline
\end{tabular}\\
\end{center}
\caption{$\Sigma$ Statistics }
\label{tab:knowngal}
\end{table*}




==> tables/knowngalv2.tex <==
\begin{table*}
\begin{center}
{Known Galaxies}\\
\begin{tabular}{cccccccccc}
\hline
\hline

Sample		&\vline& N		& Sum \ha~Flux		&\vline& N 			& Sum \ha~Flux		&\vline& N				& Sum \ha~Flux 	      		\\
 		&\vline& (\#)		& (erg/s/cm$^2$)	&\vline& (\#)			& (erg/s/cm$^2$)	&\vline& (\#)				& (erg/s/cm$^2$)		\\
		&\vline& (no cut)	& (no cut)			&\vline& (EW$>$7.5~\AA)		& (EW$>$7.5~\AA)	&\vline& (EW$>$7.5~\AA,mag$<$18)	& (EW$>$7.5~\AA,mag$<$18)	\\
		&\vline&(N,\% of N)	& (Flux,\% of Flux)	&\vline& (N,\% of N)		& (Flux,\% of Flux)	&\vline& (N,\% of N)			& (Flux,\% of Flux)		\\
\hline
All 		&\vline& 1226		& 4.15e-12		&\vline& 504			& 3.89e-12		&\vline& 346				& 3.58e-12			\\
\hline
$\Sigma\geq2.5$&\vline&297~(24.2\%)	&3.36e-12~(80.9\%)	&\vline&262~(52.0\%)		&3.32e-12~(85.2\%)	&\vline&236~(68.2\%)			&3.19e-12~(89.3\%)		\\  
$\geq$3.0	&\vline&261~(21.3\%)	&3.26e-12~(78.4\%)	&\vline&234~(46.4\%)		&3.22e-12~(82.7\%)	&\vline&216~(62.4\%)			&3.12e-12~(87.2\%)		\\
$\geq$4.0	&\vline&194~(15.8\%)	&2.96e-12~(71.1\%)	&\vline&181~(35.9\%)		&2.95e-12~(75.7\%)	&\vline&172~(49.7\%)			&2.88e-12~(80.5\%)		\\
$\geq$5.0	&\vline&152~(12.4\%)	&2.76e-12~(66.4\%)	&\vline&143~(28.4\%)		&2.75e-12~(70.7\%)	&\vline&139~(40.2\%)			&2.71e-12~(75.7\%)		\\
$\geq$6.0	&\vline&121~(~9.9\%)	&2.57e-12~(61.9\%)	&\vline&113~(22.4\%)		&2.57e-12~(65.9\%)	&\vline&112~(32.4\%)			&2.55e-12~(71.3\%)		\\
$\geq$7.0	&\vline&103~(~8.4\%)	&2.35e-12~(56.6\%)	&\vline& 97~(19.2\%)		&2.35e-12~(60.4\%)	&\vline& 96~(27.7\%)			&2.34e-12~(65.3\%)		\\
\hline
\end{tabular}\\
\end{center}
\input{tables/knowngal.txt}
%\caption{$\Sigma$ Statistics }
\label{tab:knowngal}
\end{table*}


==> tables/knowngalv3.tex <==
\begin{table*}
\begin{center}
{Known Galaxies}\\
\begin{tabular}{cccccccc}
\hline
\hline

Sample		&\vline& N		& Sum \ha~Flux		&\vline& N 			& Sum \ha~Flux		\\
 		&\vline& (\#)		& (erg/s/cm$^2$)	&\vline& (\#)			& (erg/s/cm$^2$)	\\
		&\vline&        	&           		&\vline& (EW$>$7.5~\AA)		& (EW$>$7.5~\AA)	\\
		&\vline&(N,\% of N)	& (Flux,\% of Flux)	&\vline& (N,\% of N)		& (Flux,\% of Flux)	\\
\hline
All 		&\vline& 1226		& 4.15e-12		&\vline& 504			& 3.89e-12		\\
\hline
$\Sigma\geq2.5$	&\vline&297~(24.2\%)	&3.36e-12~(80.9\%)	&\vline&262~(52.0\%)		&3.32e-12~(85.2\%)	\\  
$\geq$3.0	&\vline&261~(21.3\%)	&3.26e-12~(78.4\%)	&\vline&234~(46.4\%)		&3.22e-12~(82.7\%)	\\
$\geq$4.0	&\vline&194~(15.8\%)	&2.96e-12~(71.1\%)	&\vline&181~(35.9\%)		&2.95e-12~(75.7\%)	\\
$\geq$5.0	&\vline&152~(12.4\%)	&2.76e-12~(66.4\%)	&\vline&143~(28.4\%)		&2.75e-12~(70.7\%)	\\
$\geq$6.0	&\vline&121~(~9.9\%)	&2.57e-12~(61.9\%)	&\vline&113~(22.4\%)		&2.57e-12~(65.9\%)	\\
$\geq$7.0	&\vline&103~(~8.4\%)	&2.35e-12~(56.6\%)	&\vline& 97~(19.2\%)		&2.35e-12~(60.4\%)	\\
\hline
\end{tabular}\\
\end{center}
\input{tables/knowngal.txt}
\label{tab:knowngal}
\end{table*}


==> tables/sigexpV3.tex <==
\begin{table*}
\begin{center}
{Color Excess ($\Sigma$) Statistics}\\
\begin{tabular}{cccccc}
\hline
\hline

$\Sigma$	& N Total	& N Stars	& N High-z		& N in Correct		\\
		& Candidates	&		& Galaxies		& \ha~Filter		\\
(\#)		& (\#)		& (\#)		& (\#,\% of candidates)	& (\#,\% of candidates)	\\
\hline
2.5		&612		 &92		 &277~(45.3\%)  	   &217~(35.5\%)	     \\
3.0		&388		 &51		 &125~(32.2\%)  	   &196~(50.5\%)	     \\
4.0		&217		 &22		 &~39~(18.0\%)  	   &150~(69.1\%)	     \\
5.0		&153		 &12		 &~12~(~7.8\%)  	   &125~(81.7\%)	     \\
6.0		&116		 &~7		 &~~7~(~6.0\%)  	   &100~(86.2\%)	     \\
7.0		&~87		 &~4		 &~~2~(~2.3\%)  	   &~79~(90.8\%)	     \\
\hline
\end{tabular}\\
\end{center}
\caption{$\Sigma$ Statistics.  }
\label{tab:sigexp}
\end{table*}



==> tables/sigexpV4.tex <==
\begin{table*}
\begin{center}
{Color Excess ($\Sigma$) Statistics}\\
\begin{tabular}{cccccc}
\hline
\hline

$\Sigma$	& N Total	& N Stars	& N High-z		& N in Correct		\\
		& Candidates	&		& Galaxies		& \ha~Filter		\\
(\#)		& (\#)		& (\#)		& (\#,\% of candidates)	& (\#,\% of candidates)	\\
\hline
2.5		&769		 &59		 &299~(38.9\%)  	   &290~(37.7\%)	     \\
3.0		&478		 &34		 &128~(26.8\%)  	   &255~(53.3\%)	     \\
4.0		&273		 &16		 &~39~(14.3\%)  	   &194~(71.1\%)	     \\
5.0		&191		 &~9		 &~14~(~7.3\%)  	   &151~(79.1\%)	     \\
6.0		&145		 &~8		 &~~7~(~4.8\%)  	   &120~(82.8\%)	     \\
7.0		&121		 &~7		 &~~3~(~2.5\%)  	   &102~(84.3\%)	     \\
\hline
\end{tabular}\\
\end{center}
\caption{$\Sigma$ Statistics. }
\label{tab:sigexp}
\end{table*}



==> tables/sigexpV5.tex <==
\begin{table*}
\begin{center}
{Color Excess ($\Sigma$) Statistics}\\
\begin{tabular}{cccccccc}
\hline
\hline

$\Sigma$	& N Total	& N Stars	& N High-z		& N In		&\vline& N in Correct		 & N New in Correct	  \\
		& Candidates	&		& Galaxies		& Volume	&\vline& \ha~Filter		 & \ha~Filter		  \\
(\#)		& (\#)		& (\#)		& (\#,\% of candidates)	& (\#)		&\vline& (\#,\% of candidates) & (\#)		  \\
\hline
$\geq$2.5	&793		&82		 &317~(40.0\%)  	&378		&\vline&289~(36.4\%)		 &89	  \\
$\geq$3.0	&497		&53		 &134~(27.0\%)  	&297		&\vline&254~(51.1\%)		 &77	  \\
$\geq$4.0	&282		&25		 &~39~(13.8\%)  	&207		&\vline&193~(68.4\%)		 &55	  \\
$\geq$5.0	&197		&14		 &~14~(~7.1\%)  	&160		&\vline&151~(76.6\%)		 &40	  \\
$\geq$6.0	&150		&12		 &~~7~(~4.7\%)  	&124		&\vline&120~(80.0\%)		 &31	  \\
$\geq$7.0	&124		&~9		 &~~3~(~2.4\%)  	&105		&\vline&102~(82.3\%)		 &22	  \\
\hline
\end{tabular}\\
\end{center}
\input{tables/sigexp.txt}
\label{tab:sigexp}
\end{table*}


